A Structural Text-Based Scaling Model for Analyzing Political Discourse

Scaling political actors based on their individual characteristics and behavior helps profiling and grouping them as well as understanding changes in the political landscape. In this paper we introduce the Structural Text-Based Scaling (STBS) model to infer ideological positions of speakers for latent topics from text data. We expand the usual Poisson factorization specification for topic modeling of text data and use flexible shrinkage priors to induce sparsity and enhance interpretability. We also incorporate speaker-specific covariates to assess their association with ideological positions. Applying STBS to U.S. Senate speeches from Congress session 114, we identify immigration and gun violence as the most polarizing topics between the two major parties in Congress. Additionally, we find that, in discussions about abortion, the gender of the speaker significantly influences their position, with female speakers focusing more on women's health. We also see that a speaker's region of origin influences their ideological position more than their religious affiliation.

==> diagram.tex <==
\begin{figure}[!b]
	\centering
	\begin{tikzpicture}(14,10)
        \linethickness{0.075mm}
		% borders of the picture
		%\draw (7,-5) -- (7,-5) -- (7,5) -- (-7,5) -- cycle;
		\clip (-7,-6) rectangle (7,4);
        %% Plates - D, A, V, K, L
        \filldraw[fill=green!80!white, draw=green!40!black, fill opacity=0.2] (-2,4) -- (1,4) -- (1,1.5) -- (0,0.5) -- (0,-1) -- (-2,-1) -- cycle;
        \filldraw[fill=green!40!white, draw=green!40!black, fill opacity=0.2] (-2,4) -- (-2,-1) -- (0,-1) -- (0,-3) -- (-4,-3) -- (-4,-1) -- (-4,0) -- (-6,0) -- (-6,4) -- cycle;
        \filldraw[fill=blue!60!white, draw=blue!60!black, fill opacity=0.2] (4,4) -- (-1,4) -- (-1,1.5) -- (0,0.5) -- (0,-1) -- (0,-3) -- (2,-3) -- (2,-1) -- (4,-1) -- cycle;
        \filldraw[fill=red!60!white, draw=red!60!black, fill opacity=0.2] (-3.75,1) -- (3.75, 1) -- (7,-4) -- (3.5,-4) -- (1.25,-1) -- (-3.25,-1) -- (-4.75,-3) -- (-6.75,-3) -- cycle;
        \filldraw[fill=yellow!60!white, draw=yellow!60!black, fill opacity=0.2] (-6.75,2) -- (-4,2) -- (-4,-3) -- (-1,-4.5) -- (-1,-6) -- (-6.75,-6) -- cycle;
        %% Labels of the plates
        \draw (-1.5, 3.5) node {$D$};
        \draw (-5.25, 3.25) node {$A$};
        \draw (3.25, 3.25) node {$V$};
        \draw (4.6, -1.6) node {$K$};
        \draw (-6.3, -0.8) node {$L$};
        %% Nodes
        % outcomes Y + regressors X
		\draw (0,3.4) node(Y)[draw = black, rectangle, inner sep = 10pt] {$\mathbb{Y}$};
        \draw (-5,1) node(X)[draw = black, rectangle, inner sep = 10pt] {$\mathbb{X}$};
        % Poisson intensities lambda
        \draw (0,2) node(lambda)[draw = black, circle, inner sep = 7pt] {$\bm \lambda$};
        % Primary parameters
        \draw (-3,0) node(ideal)[draw = black, rectangle, rounded corners, inner sep = 7 pt] {$\bm \ideal$};
        \draw (-1,0) node(theta)[draw = black, rectangle, rounded corners, inner sep = 7 pt] {$\bm \theta$};
        \draw (1,0) node(beta)[draw = black, rectangle, rounded corners, inner sep = 7 pt] {$\bm \beta$};
        \draw (3,0) node(eta)[draw = black, rectangle, rounded corners, inner sep = 7 pt] {$\bm \eta$};
        % Other auxiliary parameters
        \draw (-5,-2) node(iota)[draw = black, circle, inner sep = 7pt] {$\bm \iota$};
        \draw (-3,-2) node(I)[draw = black, circle, inner sep = 7pt] {$\bm I^2$};
        \draw (-1,-2) node(btheta)[draw = black, circle, inner sep = 7pt] {$\bm b_\theta$};
        \draw (1,-2) node(bbeta)[draw = black, circle, inner sep = 7pt] {$\bm b_\beta$};
        \draw (3,-2) node(rho)[draw = black, circle, inner sep = 7pt] {$\bm \rho^2$};
        \draw (5,-3) node(brho)[draw = black, circle, inner sep = 7pt] {$\bm b_\rho$};
        \draw (-6,-4) node(iotamean)[draw = black, circle, inner sep = 7pt] {$\bm \iota_\bullet$};
        \draw (-4,-4) node(omega)[draw = black, circle, inner sep = 7pt] {$\bm \omega^2$};
        \draw (-2,-5) node(bomega)[draw = black, circle, inner sep = 7pt] {$\bm b_\omega$};
        %% Directions
        \draw [->] (lambda) -- (Y);
        \draw [->] (ideal) -- (lambda);
        \draw [->] (theta) -- (lambda);
        \draw [->] (beta) -- (lambda);
        \draw [->] (eta) -- (lambda);
        \draw [->] (iota) -- (ideal);
        \draw [->] (I) -- (ideal);
        \draw [->] (X) -- (ideal);
        \draw [->] (btheta) -- (theta);
        \draw [->] (bbeta) -- (beta);
        \draw [->] (rho) -- (eta);
        \draw [->] (iotamean) -- (iota);
        \draw [->] (omega) -- (iota);
        \draw [->] (bomega) -- (omega);
        \draw [->] (brho) -- (rho);
        
    \end{tikzpicture}
	\caption{\label{fig:hierarchy_TBIP} 
		Diagram depicting the hierarchy of the proposed extended TBIP model. Observed data (rectangles), original TBIP parameters (rounded corners), additional parameters (circles). Colored planes mark the specificity towards document ($D$), author ($A$), vocabulary ($V$), topic ($K$) and covariate ($L$).
	}
\end{figure} 

==> sec01_intro.tex <==
\section{Introduction} \label{sec:introduction}
%% just some notes:
Textual communication serves as a fundamental conduit for human expression, encapsulating a diverse spectrum of beliefs, ideologies, and perspectives. The authors' positions articulated directly or indirectly within textual content are not static but rather dynamic constructs that evolve, adapt, and vary across individuals and contexts. 
Especially in the field of political science, estimating political positions -- often called ideal points -- of political
key actors has a long tradition. Originally building up on lawmakers voting behaviour, \citet{Poole:1985} proposed a ``scaling procedure'' which provides
estimates of ideological positions of lawmakers based on their voting.
In recent years, statistical text analysis has emerged as a promising alternative method for discerning ideological stances within political discussions. This approach enables the comparison of groups that do not vote together, such as judges serving on different state courts. In addition, this approach remains applicable even when voting records are unavailable.
The pioneering \emph{Wordscore} model, as introduced by \citet{laver_benoit_garry_2003}, marked the initial attempt to estimate author positions based on textual data. However, this model had the limitation in that it necessitated a predefined set of reference texts for its application. In response to this limitation, \citet{Slapin_2008} developed the \emph{Wordfish} model, which offered an alternative approach that did not rely on predefined reference texts.
An extension of this model, known as the \emph{Wordshoal} model, was proposed by \citet{wordshoal_2016}. The distinctive feature of \emph{Wordshoal} is its capacity to adapt the meaning and discriminatory power of specific terms across different contexts.
Building upon this line of research, \citet{Vafa_etal_2020} introduced the text-based ideal point (TBIP) model, which extends the capabilities of the \emph{Wordshoal} model. One of the notable advantages of TBIP is that it does not require a prior grouping of texts based on debates or topics. As a result, TBIP combines elements from the class of topic models \citep[see][]{blei_etal_2003, Roberts_etal_JASA:2016, Gopalan:2014} with text-based ideal point models, enhancing its versatility and applicability in various research contexts. Hereby the author's specific ideal point is modelled as a univariate latent variable and applied to US Congress Speeches differences between those ideal points are interpreted as a degree of partisanship.
However the assumption of one latent ideal point on author level is strong and might be limiting in several ways: Firstly, ideal points might vary dependent on the context.
Secondly, external covariates like authors' religious beliefs, gender, political affiliation, geography, audience might influence the spoken words and so the ideal points. \textbf{Lit search!!}

In this paper, we introduce the structural TBIP model, which accommodates varying ideal points across different topics and characterizes ideal points through covariates. This model recognizes that (political) ideology in speech is not only topic-dependent but can also be influenced by a range of additional factors, such as gender, religious beliefs, audience context, and party affiliation. To comprehensively capture these effects, we integrate an innovative regression framework into the structural TBIP model. This allows us to incorporate variables representing gender, religious beliefs, audience characteristics, and party assignments as covariates in the analysis. By incorporating these dimensions into our model, we aim to provide a more nuanced and holistic understanding of how various factors shape and influence ideal points within the realm of political discourse, ultimately contributing to a richer and more comprehensive analysis of political ideology.
But also from a methodological point of view we contribute to the literature by...CAVI.
We apply our model to the 


This paper is 

\begin{itemize}
    \item taddy JASA cite
    \item GelmanJASA
    \item 
\end{itemize}


==> sec02_TBIP.tex <==
\section{Structural Text-Based Ideal-Point Model} \label{sec:STSM}

\textcolor{red}{LDA, STM, other models \ldots}

The Structural Text-Based Ideal-Point Model (STBIP) builds on and extends the Text-Based Ideal Point (TBIP) model introduced by~\citet{Vafa_etal_2020}. The TBIP model combines ideas from ideal point models for multivariate binary data that introduce a univariate latent person-specific variable (an ideal point) to account for associations between variables with the Poisson factorization framework for modeling text data. Applying TBIP to the Senate speeches in the 114th Congress, \citet{Vafa_etal_2020} infer ideological positions of the Senators that show high congruence with party membership.

STBIP extends TBIP with respect to the following aspects:
\begin{enumerate}[label=\alph*)]
    \item we allow for topic-specific ideal points to increase flexibility,
    \item we incorporate known author-level covariates in a~regression model of the ideal points, \item we propose hierarchically well-structured prior distributions.
\end{enumerate}

First, we clarify notation. We assume a~corpus of $D$ documents (speeches) and a~vocabulary of $V$ terms (bigrams) are given. A document-term matrix $\mathbb{Y}$ of shape $D \times V$ contains the frequency counts $y_{dv}$, i.e., the number of appearances of term $v \in \{1, \ldots, V\}$ in document $d \in \{1, \ldots, D\}$. $\mathbb{Y}$ is a sparse matrix, because the most frequent element of the document-term matrix is zero
given that both $D$ and $V$ are usually in the thousands and speeches are rather short. There are $A$ authors of the speeches, and $a_d \in \{1, \ldots, A\}$ indicates the author of document $d$. 

The elements $y_{dv}$ of $\mathbb{Y}$ are independently distributed Poisson counts, i.e., 
\begin{equation}\label{eq:Pois_counts}
    y_{dv} \sim \Pois{\lambda_{dv}} 
    \qquad \text{where} \qquad 
    \lambda_{dv} = \sum\limits_{k=1}^K \lambda_{dkv}
    \qquad \text{and} \qquad
    \lambda_{dkv} = \theta_{dk} \beta_{kv} \exp\{\eta_{kv} \ideal_{a_d k}\},
\end{equation}
where $K$ is the number of latent topics.

Positive per-document topic intensities $\theta_{dk}$ reflect the contribution of latent topic~$k$ to the frequency counts of speech~$d$. The term intensities of each topic for author $a_d$ are given by $\beta_{kv} \exp\{\eta_{kv} \ideal_{a_d k}\}$. Different from the original TBIP model, we assume that each author~$a$ has ideological positions $\ideal_{ak}$ specific to each topic. For an author~$a$ with latent ideal position $\ideal_{ak} = 0$ towards topic~$k$, the term intensities are captured solely by the intensities $\beta_{kv}$. Hence, we refer to them as \emph{neutral} term intensities. An ideologically shifted author~$a$ with $\ideal_{ak} \neq 0$ towards topic~$k$ has the neutral term intensities multiplied by the \emph{ideological factor} $\exp \{ \eta_{kv} \ideal_{ak} \}$ where $\eta_{kv}$ are the corresponding \emph{ideological corrections} for a unit change in ideological position $\ideal_{ak}$. Note the possible reparametrization $\eta_{kv} \ideal_{ak} = (- \eta_{kv}) (- \ideal_{ak})$ that brings identifiability issues. Hence, prior to the analysis the meaning of having a positive position has to be fixed.

\textcolor{red}{A paragraph explaining the relationship between $\eta$ and $\ideal$. Supported by some specific example. }

Speeches and authors may differ in their verbosity. To prevent that the ideal points capture differences in verbosity between authors, \citet{Vafa_etal_2020} multiplied the Poisson rate $\lambda_{dv}$ with a fixed \emph{verbosity} term specific to each author. We propose a~more flexible approach inspired by scalable Poisson factorization \citep{gopalanhofmanblei2015scalableHPoisF} where a~hierarchical prior for the intensities is used. In TBIP, the document intensities are assumed to be a-priori gamma-distributed with fixed hyperparameters, e.g., $\theta_{dk} \sim \gammadist{0.3}{0.3}$. We extend this to account for differences in speech length by using the more flexible specification with fixed shape $a_\theta$ and latent auxiliary rates 
$b_{\theta a}$ specific to each author~$a$, i.e., $\theta_{dk} \sim \gammadist{a_\theta}{b_{\theta a_d}}$, which allows for different verbosity among the authors. The latent auxiliary rates $b_{\theta a}$ are additional model parameters with prior $b_{\theta a} \sim \gammadist{a_\theta'}{\frac{a_\theta'}{b_\theta'}}$ where both hyperparameters are fixed.
%$b_{\theta d}$, i.e., $\theta_{dk} \sim \gammadist{a_\theta}{b_{\theta d}}$. The latent auxiliary rates $b_{\theta d}$ are additional model parameters with prior $b_{\theta d} \sim \gammadist{a_\theta'}{\frac{a_\theta'}{b_\theta'}}$ where both hyperparameters are fixed. 

In a similar way, we also impose a hierarchical prior structure on the neutral word intensities $\beta_{kv}$ in order to be able to capture differences in the frequency of term usage. The simple gamma prior with fixed hyperparameters is exteneded to a gamma prior with flexible $v$-rates, i.e., $\beta_{kv} \sim \gammadist{a_\beta}{b_{\beta v}}$ and $b_{\beta v} \sim \gammadist{a_\beta'}{\frac{a_\beta'}{b_\beta'}}$. For example, the bigram ``united states'' might be very popular in any of the considered topics, which would be captured by a lower rate $b_{\beta v}$.

We assume that the vast majority of terms are neutral for a given topic and only a few terms are crucial to express ideology. Therefore, we propose to use a~shrinkage prior for the ideological corrections $\eta_{kv}$. This induces a distribution with a spike at zero different from the simple $\norm{0}{1}$ distribution. We achieve this by adjusting the precision parameter $\rho_k^2$ for the normal distribution and imposing a~gamma prior. We strengthen the shrinkage by adding yet another level to the hierarchical prior distribution by imposing a prior on the rate of the gamma prior:
\begin{equation}\label{eq:prior_eta}
    \eta_{kv} \sim \norm{\mu_{\eta kv}}{\left(\rho_k^2\right)^{-1}} 
	\quad \text{with} \quad 
	\rho_k^2 \sim \gammadist{a_\rho}{b_{\rho k }}
	\quad \text{and} \quad 
	b_{\rho k } \sim \gammadist{a_\rho'}{\frac{2}{\kappa_\rho^2} \frac{a_\rho'}{a_\rho}}.
\end{equation}
This implies a very flexible prior structure which is under $\mu_{\eta kv} = 0$ equivalent to the triple gamma prior by \citet{CadonnaFruehwirth-SchnatterKnaus_triple_gamma:2019}:
\begin{equation}\label{eq:prior_triple_gamma}
    \eta_{kv}^2 \sim \gammadist{\frac{1}{2}}{\frac{1}{2\sigma_k^2}}
    \; \text{and} \;
    \sigma_k^2 \sim \gammadist{a_\rho'}{\frac{a_\rho' b_{\rho k}}{2}}
    \; \text{and} \;
    b_{\rho k} \sim \gammadist{a_{\rho}}{\frac{a_{\rho}}{\kappa_\rho^2}},
\end{equation}
where the prior structure is based on the variances $\sigma_k^2 = \left(\rho_k^2\right)^{-1}$ instead of the precisions. With $a_\rho'<1$, the marginal density has a spike at zero and $b_{\rho k}$ controls the amount of shrinkage, see \citet{Bitto_Fruehwirth-Schnatter_double_gamma:2019}. The triple-gamma prior makes the shrinkage flexible for each topic by having $b_{\rho k}$ specific for each $k$. The expected value $\E b_{\rho k} = \kappa_\rho^2$ is fixed. However, a high value of $b_{\rho k}$ induces that this topic is completely shrunken towards zero, i.e., no ideological corrections are needed for this topic. By contrast, a low value of $b_{\rho k}$ induces a non-negligible probability of obtaining $\eta_{kv}$ values far from zero. 

The last remaining parameter to be discussed are the ideological positions $\ideal_{ak}$. \citet{Vafa_etal_2020} did not include any apriori available information about the authors in the model. This allowed them to reveal in an unsupervised way that the estimated ideological positions show a high congruence with party membership. We propose to include the party membership information in the model and estimate a parameter indicating the effect of party membership on the ideological position. This also allows for the inclusion of further author-specific covariates (gender, generation, \ldots) which may impact the ideological position. We replace the independent standard normal prior with the following regression setting:
\begin{equation} \label{eq:prior_ideal}
    \ideal_{ak} \sim \norm{\T{\bm x_a} \bm \iota_k}{\left(I_a^2\right)^{-1}}
    \quad \text{and} \quad
    I_a^2 \sim \gammadist{a_I}{b_I},
\end{equation}
where $\bm x_a$ is the covariate vector of length $L$ specific to author~$a$, $\bm \iota_k$ are the regression coefficients specific to topic~$k$ and $I_a^2$ are the author-specific precisions reflecting how close the author-specific ideal points are across the topics to the predicted ideal points given the covariates. 

The topic-specificity of regression coefficients $\bm \iota_k$ implies that covariate effects may differ across topics. For example, gender might not impact word choice for most topics but when it comes to discussing women rights clear differences in word usage might be induced by gender. This feature allows us to not only identify how the covariates impact the ideal points in general but also to determine which topics are influenced the most by specific covariates. To capture the overall effect of a covariate on the ideal points, we use the following prior structure:
\begin{equation}\label{eq:prior_iota}
    \iota_{kl} \sim \norm{\iota_{\bullet l}}{\left(\omega_l^2\right)^{-1}} 
    \qquad \text{and} \qquad
    \iota_{\bullet l} \sim \norm{0}{1},
\end{equation}
where the centrality parameters $\iota_{\bullet l}$ express the aggregated effect of covariate $l \in \{1, \ldots, L\}$ and $\omega_l^2$ are the precisions which are specific to each covariate. The lower the precision, the more does the effect of this covariate differ across topics. Based on the assumption that the majority of the topics share a very similar effect of the covariate and only few topics substantially differ for covariates, we impose again the triple gamma prior~\eqref{eq:prior_triple_gamma} yielding:
\begin{equation}\label{eq:prior_omega}
    \omega_l^2 \sim \gammadist{a_\omega}{b_{\omega l}}
    \qquad \text{and} \qquad 
    b_{\omega l} \sim \gammadist{a_\omega'}{\frac{2}{\kappa_\omega} \frac{a_\omega'}{a_\omega}}.
\end{equation}
In this case the shrinkage of the coefficients is not necessarily towards zero, but to the centrality parameters $\bm \iota_{\bullet l}$.

The hierarchy of the extended TBIP model is depicted in Figure~\ref{fig:hierarchy_TBIP}.
\input{JASA_paper/diagram2}



==> sec04_senate.tex <==
\section{US congress - senate speeches} \label{sec:senate}

We apply our hierarchical version of TBIP to the U.S.\ Senate speeches dataset \citep{Taddy_etal_2019, Vafa_etal_2020}, focusing on the 114th Congress session (2015\,--\,2017) as our predecessors. First, we compare the results of the original TBIP model to our hierarchical version of TBIP with a single covariate representing party membership. Then, we extend the regression analysis to other covariates potentially effecting the ideological position. Note that our model specification only allows for author-specific covariates in the regression. 

The Congression Record provided by~\citet{Gentzkow+Shapiro+Taddy:2018} also contains the information about the gender of the senators and for which state they were elected. \citet{Skelley2023} provides information on the age and years of service for each Congress member\footnote{Freely available at Github: \url{https://github.com/fivethirtyeight/data/tree/master/congress-demographics}.}. Moreover, Pew Research Center provides a~database on the religious affiliations \footnote{\url{https://www.pewresearch.org/religion/2015/01/05/members-of-congress-religious-affiliations/}}. 
\textcolor{red}{Improve the citations.}

We limit the analysis to speeches in the Senate given by Senators in active service. Out of 100 Senators, we keep $99$ Senators who made more than 24 speeches. We use the same list of stop words as \citet{Vafa_etal_2020} and follow their data pre-processing procedure that utilizes the \texttt{CountVectorizer} function from \texttt{scikit-learn} package \citep{scikit-learn}. We only keep the bigrams (not unigrams or trigrams) that appear in at least 0.1\% and at most 30\% of documents. We also keep bigrams used by 10 or more Senators to eliminate the terms used only by a~small number of Senators.  This results in $D=14\,672$ non-empty speeches containing $V=5\,031$ terms. The choice of the number of topics follows  \citet{Hofmarcher+Adhikari+Gruen:2022} who add 3 topics to the 22 topics used in~\citet{Gentzkow_etal_2019}, which were manually predefined to capture the content in Congress speeches in a suitable way. Hence, $K=25$ is used in analyses below. Moreover, in all applications we initialize the variational parameters $\phi_\theta$ and $\phi_\beta$ with the same corresponding outputs of hierarchical Poisson factorization with $K=25$, which more-or-less preserves the meaning of each of the topics $k \in \{1, \ldots, K\}$. 

The demographics of the 99 Senators in the 114th Congress session used in the analysis can be summarized in the following way: There are 53 Republicans and 44 Democrats, the remaining 2 are independent Senators. The Senate is dominated by men (79 out of 99). Dividing the USA into 5 regions, we obtain the following counts: Midwest (25), West (25), Northeast (21), Southeast (18) and South (10). \citet{Skelley2023} points out that the Congress gets older than ever, which is in line with the generation composition: Silent generation (1928--1945, 22 senators), Boomers (1946--1964, 62 senators) and Gen X (1965--1980, 15 senators). 13 Senators were newcomers to the Senate, 6 of them were even new to the Congress and 30 Senators had already served in more than 10 Congress sessions. The last considered covariate is religion which has diverse set of possibilities once the Christianity is split up according to different churches. We decided to keep all categories having at least 7 members and group the rest into one baseline category Other (18 senators: Unspecified/Other Protestant, Anglican/Episcopal, Congregationalist, Nondenominational Christian, Buddhist or those who refused to state their religion). The kept categories include: Catholic (25), Presbyterian (14), Baptist (10), Jewish (9), Methodist (9), Lutheran (7), Mormon (7).


% \paragraph{One paragraph summarizing the speech preprocessing:}
% \begin{itemize}
%    \item[\checkmark] which senators kept - more than 24 speeches
%    \item[\checkmark] stopwords
%    \item[\checkmark] which speeches kept - minimum (0.001) and maximum (0.3) document frequency
%    \item[\checkmark] bigrams only - include those used at least by 10 senators
%    \item[\checkmark] the use of \texttt{CountVectorizer} from \texttt{sklearn}
%    \item[\checkmark] final dimensions: $D$, $A$, $V$ and choice of $K$
% \end{itemize}

\begin{comment}
%%%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%               NEW SUBSECTION                   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!%%%
\subsection{Topic-specificity of ideological positions} \label{subsec:ideal_a_vs_ak}
\textcolor{red}{Only in Appendix. Main focus should be on the regression. }
\begin{enumerate}
    \item Comparison of the original TBIP model with our version with topic-specific ideological positions (without regression).
    \item Show how the positions can vary from topic to topic.
    \item Show that the original TBIP model estimates the positions quite precisely compared to the topic-specific positions in our extension
\end{enumerate}
\end{comment}


%%%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%               NEW SUBSECTION                   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!%%%
\subsection{Fixed ideological position} \label{subsec:reg_ideal_a}

Before we present the results of the proposed STBIP model we make a smaller step to examine the effect of all of the considered covariates on the unique fixed ideological positions. \citep{Vafa_etal_2020} found the strong association with the party membership which, however, does not exclude the possibility of other associations. 

We set up a~simplified STBIP where topic dimension of ideological position $\ideal$ is suppressed and just a~single regression model is assumed for them. The prior structure for regression parameters is also simplified by removing the topic dimension and unnecessary layers. For now we assume additive regression set up with several categorical covariates (baseline category): party (Democrats), gender (male), region (Northeast), generation (Silent), experience (10+ years in Congress) and religion (Other).

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{JASA_paper/fig/TBIPhier_ideal_a_Nreg_all_no_int/covariate_effects.pdf}
    \caption{Results of additive regression model built on fixed ideological positions.}
    \label{fig:TBIPhier_ideal_a_Nreg_all_no_int_covariate_effects}
\end{figure}

The results are summarized in Figure~\ref{fig:TBIPhier_ideal_a_Nreg_all_no_int_covariate_effects}. In the histogram on the top we can clearly see the strong dependence of ideological positions on party membership which is confirmed in the row below with resolutely significant CCP on the left hand side. On the same side below you can find the CCPs for testing all differences between baseline and other categories simultaneously while the traditional significance labels inside the rectangles depict the significance of comparing the corresponding single category to the baseline. The colour of those rectangles depicts the actual size of the effect. 

We can see that the experience (years served in Congress) is also significant where it seems that the newcomers tend to be on the positive side of ideological spectrum. At this point we should point out that the six Freshman all come from Republican party which suggests proper specification by interaction terms. Very similar statement could be said about region where we can suppose different speech tendencies for Democrats and Republicans in each region. It seems that some Christian churches (Presbyterian, Baptist) tend to be more positive on the ideological spectrum but that is on the edge of significance. Gender and generation do not seem significant at all.

However, all of that can change once we suppose topic-specificity of ideological positions. We hope to find topics for which even insignificant covariates (like gender) may be relevant. Moreover, by comparing the effect sizes we can determine which topics the party membership effects the ideological position the most and the least.

%\textit{Author verbosities vs author specific rates for theta?}


%%%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%               NEW SUBSECTION                   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!%%%
\subsection{Topic-specific ideological positions, party covariate only} \label{subsec:topics_party}

\textit{Adept for an appendix, but for now keep here. If so, include Fig 3 for model from section 4.3 where we display ideological positions and colour by party + crosses made by averaging across party.}

In this section, we apply our full STBIP model on the senate speech data but with party covariate only. We leave the detailed regression analysis for the next section. This allows us to fully concentrate on the effect of party and map the discrepancy in various topics. This is possible through topic-specific ideological positions that are assumed in our STBIP.

We also compare our results to the original TBIP model by~\citep{Vafa_etal_2020} applied to our dataset. Their specification counts with fixed ideological positions and simple fixed prior distributions. Nevertheless, they are rightfully proud for clear separation of Democrats and Republicans on ideological space despite any use of the party covariate within the model. The corresponding ideological positions by TBIP can be found in the first line of Figure~\ref{fig:ideal_points_hier_vs_TBIP_party_by_iota_K25} where the crosses connected by line show the party means.  

\begin{figure}
    \centering
    \includegraphics[width=0.87\textwidth]{JASA_paper/fig/ideal_points_hier_vs_TBIP_party_by_iota_K25.png}
    \caption{Topic-specific ideal points compared to topic-invariant ideological positions estimated by classical TBIP:
    Democrats (blue), Republicans (red), Independent (grey). 
    %Democrats (lightblue) are represented by Charles Schumer (blue) and Republicans (orange) are represented by Mitch McConnell (red). 
    Black lines connect the estimated locations with regression coefficients for Democrats and Republicans. Topics are ordered by the distance between them.}
    \label{fig:ideal_points_hier_vs_TBIP_party_by_iota_K25}
\end{figure}

Other rows of Figure~\ref{fig:ideal_points_hier_vs_TBIP_party_by_iota_K25} depict the ideological positions from STBIP. They are ordered by the distance between party means estimated  by the regression coefficients. With Democrats as baseline this difference is directly (an absolute value of) one of the regression coefficients for which we have a posterior approximation by (an absolute value of) normal distribution. Therefore, no post-processing is required to evaluate the discrepancy between parties, it is already included in the model specification. We ordered the topics with respect to the size of this effect. Hence, on the top of the plot we can find topics for which Democrats and Republicans differ the most, while the bottom contains topics where the party membership seems not to effect the ideology on the topic. 

For example, topic~5 is dedicated to guns and violence according to wordclouds in Figure~\ref{fig:TBIPhier_all_wordclouds_logscale_selected_topics}. While a senator of extremely negative ideological position (-1, a Democrat most likely) would rather do a background check including psychological evaluation of mental health before allowing to use a gun, a senator of extremely positive ideological position (1, a Republican most likely) would rather prevent the gun violence with anti-terrorist precautions focusing on radical islamic citizens. On the other hand, when it comes to health services (topic~9) both parties seem to be equally inclined towards negative positions that rather focuses on the medical care for veterans. However, in both parties we can find senators that rather highlight health and medical care from legislative point of view. 

\begin{figure}
    \centering
    \includegraphics[width=0.97\textwidth]{JASA_paper/fig/TBIPhier_all/wordclouds_logscale_selected_topics.png}
    \caption{Wordclouds for selected topics. The top 10 terms are determined based on the variational mean of $\bm \beta$ (on log-scale) corrected by the ideological term under: negative ($\mathsf{i}=-1$), neutral ($\mathsf{i}=0$) and positive ($\mathsf{i}=1$) ideological position.}
    \label{fig:TBIPhier_all_wordclouds_logscale_selected_topics}
\end{figure}

Using the weights $w_{ak}$ defined in Section~\ref{subsec:inference} we reduced the ideological positions into a weighted average. These aggregated positions ('WghtAvrg' in Figure~\ref{fig:ideal_points_hier_vs_TBIP_party_by_iota_K25}) were compared to the ideal points from the original TBIP model and Pearson's correlation coefficient exceeded 0.9, which proves that despite the assumed diversification of ideological positions the overall ideology is preserved. 

%To quantify the correspondence between our results and the original TBIP model we averaged ideological positions across topics and computed Pearson's correlation coefficient. However, we realized that we should respect the profoundness of each topic so that the ideological positions of highly discussed topics have higher weight. Therefore, we computed the variational means of $\theta_{dk}$, averaged them over documents of each author and then used them as weights to create a unifying ideological position for each author. In Figure~\ref{fig:ideal_points_hier_vs_TBIP_party_by_iota_K25} the row 'WghtAvrg' displays those final ideological positions which reach a correlation slightly higher than 0.9 with the ideological positions from the original TBIP. 

The effect of the change from fixed ideological positions to topic-specific ones pervades through many layers of our model. For example, consider the ideological corrections $\eta_{9v}$ with their prior precisions $\rho_9^2$ for topic~9 for which the main parties do not seem to differ in ideology. When the ideological position is common to all topics the precision is the highest of all the topics which shrinks the corrections towards zero so that the highly party related positions do not mislead the ideological term. On the other hand, with topic-specific ideological positions the variational mean of $\rho_9^2$ becomes the second lowest among all topics which yields high variability in the corrections $\eta_{kv}$ that are now tied with more appropriate ideological positions.

\begin{comment}
Explain what exactly do you mean by the original TBIP. 

\begin{itemize}
    \item Application of the hierarchical model including the author-level regression (BUT political party only!).
    \item Comparing averaged topic-specific locations to positions from original TBIP by party (could be also in previous subsection).
    \item[\checkmark] Plot the verbosities from classical TBIP against the author-specific prior rates for $\bm \theta$. 
    \item[\checkmark] Plot the differences between Democrats and Republicans in each topic.
    \item[\checkmark] Show the wordclouds for topics with the highest (and lowest) discrepancy between parties.
    \item[?] Show short quotations from the most influential speeches.
\end{itemize}


\begin{figure}    \centering
    \includegraphics[width=\textwidth]{JASA_paper/fig/verbosities_TBIP_vs_Garte_K25.png}
    \caption{Comparison of author verbosities estimated under the classical TBIP model and author-specific rates for document intensities $\theta$ (on log-scale).}
    \label{fig:verbosities_TBIP_vs_Garte_K25}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{JASA_paper/fig/ideal_points_hier_vs_TBIP_party_by_average_K25.png}
    \caption{Topic-specific ideal points compared to topic-invariant ideological positions estimated by classical TBIP. Democrats (lightblue) are represented by Charles Schumer (blue) and Republicans (orange) are represented by Mitch McConnell (red). Black lines connect the party means, topics are ordered by the distance between them.}
    \label{fig:ideal_points_hier_vs_TBIP_party_by_average_K25}
\end{figure}

    \begin{figure}
        \centering
        \includegraphics[width=0.7\textwidth]{JASA_paper/fig/ideal_points_as_distribution_hier_vs_TBIP_party_by_average_K25.png}
        \caption{Mixture distributions of topic-specific ideal points compared to topic-invariant ideological positions estimated by classical TBIP. Topics are ordered by the distance between Democrats (blue) and Republicans (red). Black lines connect the party means.}
        \label{fig:ideal_points_as_distribution_hier_vs_TBIP_party_by_average_K25}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.7\textwidth]{JASA_paper/fig/ideal_points_as_distribution_hier_vs_TBIP_party_by_iota_K25.png}
        \caption{Mixture distributions of topic-specific ideal points compared to topic-invariant ideological positions estimated by classical TBIP. Topics are ordered by the distance between Democrats (blue) and Republicans (red). Black lines connect the estimated party locations with regression coefficients.}
        \label{fig:ideal_points_as_distribution_hier_vs_TBIP_party_by_iota_K25}
    \end{figure}
    
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{JASA_paper/fig/ideal_points_as_distribution_best_worst_hier_vs_TBIP_party_by_average_K25.png}
    \caption{Mixture distributions of topic-specific ideal points compared to topic-invariant ideological positions estimated by classical TBIP. Topics are ordered by the distance between Democrats (blue) and Republicans (red), only 5 topics with the highest and lowest difference are shown. Black lines connect the party means.}
    \label{fig:ideal_points_as_distribution_best_worst_hier_vs_TBIP_party_by_average_K25}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{JASA_paper/fig/ideal_points_as_distribution_best_worst_hier_vs_TBIP_party_by_iota_K25.png}
    \caption{Mixture distributions of topic-specific ideal points compared to topic-invariant ideological positions estimated by classical TBIP. Topics are ordered by the distance between Democrats (blue) and Republicans (red), only 5 topics with the highest and the lowest difference are shown. Black lines connect the estimated party locations with regression coefficients.}
    \label{fig:ideal_points_as_distribution_best_worst_hier_vs_TBIP_party_by_iota_K25}
\end{figure}

\begin{figure}
    \centering
    %\includegraphics[width=0.97\textwidth]{JASA_paper/fig/hierparty_top5_party_wordclouds_logscale_K25.png}
    \includegraphics[width=0.97\textwidth]{JASA_paper/fig/party_only_top5_party_wordclouds_logscale_K25.png}
    \caption{Wordclouds of the most party distinguishing topics based on estimated regression coefficients. Neutral correspond to the variational mean of objective topics $\bm \beta$. Positive and negative columns correspond to the variational mean of $\bm \beta$ multiplied by variational mean of the ideological term given ideological position equal to 1 or $-1$, respectfully.}
    \label{fig:hierparty_top5_party_wordclouds_logscale_K25}
\end{figure}

\begin{figure}
    \centering
    %\includegraphics[width=0.97\textwidth]{JASA_paper/fig/hierparty_tail5_party_wordclouds_logscale_K25.png}
    \includegraphics[width=0.97\textwidth]{JASA_paper/fig/party_only_tail5_party_wordclouds_logscale_K25.png}
    \caption{Wordclouds of the topics that differ between Democrats and Republicans the least based on estimated regression coefficients. Neutral correspond to the variational mean of objective topics $\bm \beta$. Positive and negative columns correspond to the variational mean of $\bm \beta$ multiplied by variational mean of the ideological term given ideological position equal to 1 or $-1$, respectfully.}
    \label{fig:hierparty_tail5_party_wordclouds_logscale_K25}
\end{figure}
\end{comment}

%%%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%               NEW SUBSECTION                   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!%%%
\subsection{Detailed regression analysis} \label{subsec:detailed_regression}

\textit{This section is written under the assumption that 4.2 is not present here, but maybe in the Appendix.}
\begin{comment}
Our story flow
\begin{enumerate}
    \item Maybe, party is not the only relevant covariate determining the liberality/conservativeness. Show results on TBIP with fixed positions for all topics no interactions, Figure~\ref{fig:TBIPhier_ideal_a_Nreg_all_no_int_covariate_effects}.
    Some may seem irrelevant, however, suggest:
    \begin{enumerate}
        \item interaction with party so that the effects can be party-specific (region),
        \item topic-specificity of the ideological positions.
    \end{enumerate}
    \item What happens when interactions are added but not topic-specificity, Figure%~\ref{fig:TBIP_ideal_a_reg_with_interactions_party_effects_interactions}.
    \item Ideological-positions topic-specific:
    \begin{enumerate}
        \item P-values heatmaps for effects of Democrats and Republicans, Figure%~\ref{fig:TBIPhier_all_pvalues_table}.
        \item Suddenly, region becomes very important for all topics. The same story for generation effect for Democrats. 
        \item Topic 13: significant gender effect for both parties, see Figure~\ref{fig:TBIPhier_all_party_effects_interactions_k_13}.
        \item Topic 14: significant experience effect for Republicans who have 6 newcomers to the Senate while Democrats have none, see Figure~\ref{fig:TBIPhier_all_party_effects_interactions_k_14}.
        \item Topic 15: significant difference between Presbyterian and Mormon in Democratic party, see Figure~\ref{fig:TBIPhier_all_party_effects_interactions_k_15}.
        \item Wordclouds in the Appendix, Figures~\ref{fig:TBIPhier_all_wordclouds_logscale_topics_0_4}, 
        \ref{fig:TBIPhier_all_wordclouds_logscale_topics_5_9}, 
        \ref{fig:TBIPhier_all_wordclouds_logscale_topics_10_14},
        \ref{fig:TBIPhier_all_wordclouds_logscale_topics_15_19},
        \ref{fig:TBIPhier_all_wordclouds_logscale_topics_20_24}.
    \end{enumerate}
\end{enumerate}
\end{comment}

In this section, we apply the STBIP model with topic-specific ideological positions to the senate speech data with all covariates as in Section~\ref{subsec:reg_ideal_a}. However, this time we even include the interaction terms of all covariates with party, which allows us to evaluate the effects of all covariates for all parties separately. One of the advantages of our structural modelling is that the complex prior distribution allows to work with coefficients that would be otherwise unidentifiable (e.g. no Democratic Freshman or interactions with only two Independent senators). 

Figure~\ref{fig:ideal_points_hier_vs_TBIP_party_by_weighted_average_K25} displays the estimated ideological positions for all $K=25$ topics. The Democratic (blue) and Republican (red) averages marked by crosses are actually weighted by $w_{ak}$ defined in Section~\ref{subsec:inference}. % variational means of $\theta_{dk}$ averaged across documents for all authors separately. 
To quantify the correspondence between our results and the original TBIP model we averaged ideological positions across topics and computed Pearson's correlation coefficient with the ideological positions from the original TBIP which reaches almost 0.9. 
This proves that despite the assumed diversification of ideological positions the overall ideology is preserved. 

We have ordered the topics with respect to the distance between Democrats and Republicans to determine the topics for which party membership effects the ideological position the most. 
For example, topic~5 is dedicated to guns and violence according to wordclouds in Figure~\ref{fig:TBIPhier_all_wordclouds_logscale_selected_topics}. While a senator of extremely negative ideological position (-1, a Democrat most likely) would rather do a background check including psychological evaluation of mental health before allowing to use a gun, a senator of extremely positive ideological position (1, a Republican most likely) would rather prevent the gun violence with anti-terrorist precautions focusing on radical islamic citizens. 
%On the other hand, when it comes to health services (topic~9) both parties seem to be equally inclined towards negative positions that rather focuses on the medical care for veterans. However, in both parties we can find senators that rather highlight health and medical care from legislative point of view. 
On the other hand, when it comes to public health and universities (topic~8) both parties have speakers on both sides of ideological spectrum. Some would rather mention zika virus or pregnant women while other would rather talk about student loans and loan programs.

Christopher Murphy (Democrat, CT, 20160615, $\ideal_{\text{CM},5} \doteq -2.2$):
\textit{
\ldots They came to this Congress to argue on behalf of those still living on the streets of this country who could benefit by an expanded background check system that would stem the flow of illegal weapons on their streets. Had we been successful, had we been able to pick up a few more votes to persist and beat that filibuster, maybe Jonathan Aranda would be alive today. Had we years ago passed a law that puts people who have had an intersection with the FBI with respect to terrorist connections on the list of those who are prohibited from buying guns. Maybe that network would have caught up with Omar Mateen, and he would never have bought the weapon that he used to kill those in Orlando. 
}

Benjamin Cardin (Democrat, MD, 20160621, $\ideal_{\text{TC},5} \doteq -0.4$):
\textit{
It should not matter whether you buy a gun at a local gun store or at a gun show or on the Internet. You should have to pass a background check so we can make sure guns are kept out of the hands of people who should never have one. This amendment would have helped keep guns out of the hands of convicted felons, domestic abusers, and the seriously mentally ill, who have no business buying a gun. Studies have shown that nearly half of all current gun sales are made by private sellers who are exempt from conducting background checks.
}

Ted Cruz (Republican, TX, 20160616, $\ideal_{\text{TC},5} \doteq 1.5$):
\textit{
Our nation is at war. Five days ago, we saw a horrific terror attack in Orlando, FL. 
\ldots
Radical Islamic terrorism has declared jihad on America. As the facts have unfolded, they now indicate that the Orlando terrorist had pledged his allegiance to ISIS in the process of murdering 49 and wounding more than 50 at a nightclub.
\ldots
I have spent years defending the Second Amendment, the right to keep and bear arms, the Constitution and the Bill of Rights. And I, along with the Presiding Officer, along with a great many Members of this Chamber, am committed to defending the constitutional rights of every American. You don't defeat terrorism by taking away our guns, you defeat terrorism by using our guns.
\ldots
It is offensive to play political games with the constitutional rights of American citizens instead of getting serious about keeping this country safe.
\ldots
We need serious leadership focused on keeping this country safe. A second component of keeping this country safe is defeating ISIS utterly and completely defeating ISIS. In yesterdays circus, when calling for taking away your and my constitutional rights, how often did Senate Democrats say: Lets utterly destroy ISIS.
}

\textit{Use again topic~9 which does not have the lowest difference but mean position for Democrats is even higher than for Republicans OR use topic~8 with the lowest difference? Moreover, topic~8 does not have the same shift in $\rho_k^2$ when changing the topic-specificity of $\ideal$ as topic~9 does. }



\begin{figure}
    \centering
    \includegraphics[width=0.87\textwidth]{JASA_paper/fig/ideal_points_hier_vs_TBIP_party_by_weighted_average_K25.png}
    \caption{Topic-specific ideal points compared to topic-invariant ideological positions estimated by classical TBIP:
    Democrats (blue), Republicans (red), Independent (grey). 
    %Democrats (lightblue) are represented by Charles Schumer (blue) and Republicans (orange) are represented by Mitch McConnell (red). 
    Black lines connect the weighted averages of ideological positions for Democrats and Republicans. Topics are ordered by the distance between them.}
    \label{fig:ideal_points_hier_vs_TBIP_party_by_weighted_average_K25}
\end{figure}

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{JASA_paper/fig/TBIPhier_ideal_a_Nreg_all_no_int/covariate_effects.pdf}
    \caption{Results of additive regression model built on fixed ideological positions.}
    \label{fig:TBIPhier_ideal_a_Nreg_all_no_int_covariate_effects}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{JASA_paper/fig/TBIP_ideal_a_reg_with_interactions/party_effects_interactions.pdf}
    \caption{Results of regression model with interactions built on fixed ideological positions.}
    \label{fig:TBIP_ideal_a_reg_with_interactions_party_effects_interactions}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{JASA_paper/fig/TBIPhier_all/pvalues_table_Democrats.png}
        \caption{Democrats.}
        \label{fig:TBIPhier_all_pvalues_table_Democrats}
    \end{subfigure}
    ~
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{JASA_paper/fig/TBIPhier_all/pvalues_table_Republicans.png}
        \caption{Republicans.}
        \label{fig:TBIPhier_all_pvalues_table_Republicans}
    \end{subfigure}
    \caption{VI P-values for significance of the covariate effects subject to political party.}
    \label{fig:TBIPhier_all_pvalues_table}
\end{figure}
\end{comment}

Next, we report the results of the regression on the ideological positions. For each topic~$k$ we constructed a summarizing plot, see Figures~\ref{fig:TBIPhier_all_party_effects_interactions_k_11}, \ref{fig:TBIPhier_all_party_effects_interactions_k_13} and \ref{fig:TBIPhier_all_party_effects_interactions_k_15} for topics 11, 13, and 15, respectively. The plot is split into two halfs: left for Democrats, right for Republicans. In the top of the plot, there are histograms of the ideological positions, which display the difference in distribution between parties more clearly than Figure~\ref{fig:ideal_points_hier_vs_TBIP_party_by_weighted_average_K25}. The line below contains the estimated ideological position for a party member of baseline categories of other covariates. The p-value for party on the left side corresponds to testing the difference between these two effects. The other p-values on the left hand side correspond to testing the importance of interaction terms, that is, whether the effects of the covariates differ between the two parties. Next, p-values hidden in the rectangles dedicated to baseline categories belong to significance test of effects of all categories within the respective party. Finally, the rectangles for other categories are colored by the size of the effect compared to the baseline and contain the traditional significance labels for that effect. 

By examination of all plots we noticed that the interaction term of party and region is necessary for almost all topics. For example, while Democratic senators of Northeast and Midwest are of very comparable ideology, Republicans from Midwest tend to have more positive position than those from Northeast. On the other hand, the experience seems to be important in most of the topics but the differences in this effect between the two parties are rarely significant. Hence, interaction term of party and experience could be omitted, yet keep in mind there are no Democratic Freshmen.

Topic~11 is clearly dedicated to climate change where we could expect some ideological discrepancies between (relatively) young and old generations. And indeed, in Figure~\ref{fig:TBIPhier_all_party_effects_interactions_k_11} we observe significant effect of generation in the Democratic party where it seems that younger generation tends to have more positive ideological position. Positive extremists would rather talk about entitled oversight while negative extremists highly use 'fossil fuel' or 'carbon pollution'. 

Edward Markey (Democrat, Boomer generation, MA, 20160712, $\ideal_{\text{EM},11} \doteq -1.2$):
\textit{
Already this year there have been eight weather-related and climate-related disasters that each caused at least \$1 billion in damage. 
\ldots
James Black: "In the first place there is general scientific agreement that the most likely manner in which mankind is influencing the global climate is through carbon dioxide release from the burning of fossil fuels."
\ldots
We must take the climate deniers and their fossil fuel funders to task for their obstinate, obdurate, oblivious opposition to the clean energy to battle climate change.
}

Richard Durbin (Democrat, Silent generation, IL, 20160712, $\ideal_{\text{RD},11} \doteq -0.4$):
\textit{
Climate change is one of the greatest threats to our planet Earth. When I look at my beautiful grandkids. I feel a moral responsibility to leave this world as well as I found it or even better. We cant continue to ignore the problem of climate change. How will future generations judge us if we deny the reality of climate change and say that it is just too hard to do something that might leave them a safer. cleaner. better world? I don't think they will look on us kindly. Future generations actually count on us. Climate change is no longer debatable.
}

Shelley Capito (Republican, Boomer generation, IL, 20151117, $\ideal_{\text{SC},11} \doteq 0.2$):
\textit{
The Senate now has the chance to take a real up-or-down vote on whether the EPAs Clean Power Plan can and should move forward. This is a legal binding resolution that if successful will prevent the Clean Power Plan or a similar rule from taking effect. Passing this resolution will send a clear message to the world that a majority of the Congress does not stand behind the Presidents efforts to address climate change with economically catastrophic regulations. Passing this resolution will also demonstrate to the American people that the Senate understands the need for affordable and reliable energy.
}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{JASA_paper/fig/TBIPhier_all/party_effects_interactions_k_11.pdf}
    \caption{Results of regression model with interactions built on ideological positions for topic~11.}
    \label{fig:TBIPhier_all_party_effects_interactions_k_11}
\end{figure}


The topic~13 about planned parenthood in Figure~\ref{fig:TBIPhier_all_party_effects_interactions_k_13} has been chosen to demonstrate the significant effect of gender (p-values 0.004 and 0.001). Regardless of the party membership, women tend to have much more negative ideological position than men. From the wordclouds in Figure~\ref{fig:TBIPhier_all_wordclouds_logscale_selected_topics} we see that the speaker with negative ideological position would prefer to use terms like 'womens health', 'family planning' or 'care services' while speaker with positive ideological position would prefer to talk about 'unborn children' and 'foster care'.

Dianne Feinstein (Democrat, CA, 20150924, $\ideal_{\text{DF},13} \doteq -1.0$):
\textit{
I rise once again to speak against this callous misguided effort to defund Planned Parenthood. This is a clear case of politics being put ahead of the countrys best interests. This time the majority has tied this effort to the funding of the entire Federal Government, they are willing to shut down the government over this issue. That is preposterous. Planned Parenthood serves some of the most vulnerable women in our society. It cares for 2.7 million patients in the U.S.- million patients worldwide.
\ldots
Community health centers and clinics do great work, but if 2.7 million Planned Parenthood patients were suddenly without a doctor, they simply could not handle the sudden influx of new patients.
\ldots
We are standing up for Planned Parenthood because we stand up for women. I urge a "no" vote. Lets defeat this bill and move on so we can fund the government and address many other critical issues.
}

Kelly Ayotte (Republican, NH, 20150922, $\ideal_{\text{KA},13} \doteq -0.2$):
\textit{
An issue has come up that is a very important issue. And that is an organization called Planned Parenthood and holding Planned Parenthood accountable in the wake of deeply disturbing videos that discuss the appalling practice of harvesting the organs and body parts of unborn babies.
I was just sick to see the contents of recent videos that have been disclosed that show a callous disregard by officials at Planned Parenthood for the dignity of human life.
\ldots 
That is why last month I joined a bipartisan majority of Senators in voting to redirect Federal funding from Planned Parenthood to community health centers that provide womens health services.
\ldots
So in good conscience, while I fully support redirecting the money from Planned Parenthood to community health centers who serve women, I cannot in good conscience participate again in this process, one that would ensure we come closer to the brink of a shutdown, when I have not heard a strategy for success.
}

Ted Cruz (Republican, TX, 20150928, $\ideal_{\text{TC},13} \doteq 1.8$):
\textit{
Planned Parenthood is a private organization. It is not even part of the government. But it happens to be politically favored by President Obama and the Democrats. Planned Parenthood is also the subject of multiple criminal investigations for being caught on tape apparently carrying out a pattern of ongoing felonies.
\ldots
I am advocating that we fight on things that matter. Don't give \$500 million to Planned Parenthood, a corrupt organization that is taking the lives of vast numbers of unborn children and selling their body parts.
}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{JASA_paper/fig/TBIPhier_all/party_effects_interactions_k_13.pdf}
    \caption{Results of regression model with interactions built on ideological positions for topic~13.}
    \label{fig:TBIPhier_all_party_effects_interactions_k_13}
\end{figure}

Finally, we searched for a~topic that would distinguish the different religion beliefs the most  and topic~15 about nuclear weapons and middle east seems to be the one where the effects within Democratic party seem to be the most diverse. In Figure~\ref{fig:TBIPhier_all_party_effects_interactions_k_15} we see that Democratic Presbyterian are more positive while Mormons or Methodists tend to have more negative ideological position. In general, negative ideological position for this topic is connected with terms like 'foreign relations' and 'human rights'. On the other hand, 'Obama administration' and 'national security' is more prevalent with speakers of negative ideological position. 

Harry Reid (Democrat, Mormon, RI, 20150909, $\ideal_{\text{HR},15} \doteq -0.5$):
\textit{
It is important to note that this agreement does not take away the tools available to the President to target sanctions against Irans violation of human rights or to damage Irans ability to finance terrorism. U.S. secondary sanctions remain in place.
\ldots
These secondary sanctions are not insignificant tools, and our use of them in response to human rights violators and terrorism are not a violation of the agreement.
\ldots
I believe the JCPOA will give us valuable tools to monitor and interdict their pathways to a nuclear weapon, but it will require day-to-day surveillance and, where necessary, intervention to increase our chances of success. We have concluded an agreement that dramatically constrains Irans nuclear ambitions. Now the hard work begins each day to ensure that our aspirations become real.
}

Chris Coons (Democrat, Presbyterian, DE, 20150909, $\ideal_{\text{CC},15} \doteq 0.1$):
\textit{
I am deeply suspicious of Iran, the worlds leading state sponsor of terrorism. I am also deeply suspicious of Irans intentions for its nuclear program, given its long record of cheating on past deals and of consistently expressing virulently antiAmerican, antiSemitic and antiIsrael views.
\ldots
Scripture offers us many stories, from Genesis to Deuteronomy to Isaiah and the gospels, in which we are encouraged to pursue diplomacy before resorting to conflict. My support of this agreement in no small part is an attempt to heed that advice. We cannot trust Iran. But this deal, based on distrust, verification, deterrence and strong multilateral diplomacy, I have concluded, offers us our best opportunity to prevent a nuclear-armed Iran.
}

Orrin Hatch (Republican, Mormon, UT, 20150910, $\ideal_{\text{CC},15} \doteq 0.4$):
\textit{
Our quarrel is not with the Iranian people. The Iranian people are our friends. Instead, it is the dictatorial and fanatical regime that seeks to build and even use nuclear weapons to destabilize the entire region and to kill Americans and Israelis. Given the threat posed by this rogue regime, preventing Iran from acquiring a nuclear weapons capability is absolutely critical. It is a goal shared across party lines as well as among many of our friends and allies abroad. All of us here prefer to prevent Iran from acquiring this capability by diplomatic means if possible rather than by armed conflict. In light of this shared desire to resolve the Iranian threat without a war. I examined the Obama administrations proposed agreement hopeful, if skeptical, that I could support the agreement. Nevertheless, the duty incumbent upon us as Senators is not to accept or reject this deal based upon kneejerk reactions or blind partisan loyalty but rather to determine our stances based on thorough examination and reasoned judgment. Regrettably, after much study, I have concluded that this is a catastrophically bad deal that I must strongly oppose.
\ldots
A deal that paves rather than precludes Irans path to a nuclear weapons capability makes war more likely. A deal that makes the Iranian regime more confident of its ability to protect its nuclear program from international pressure and military action makes war more likely. A deal that funnels tens of billions of dollars to terrorists bent on destabilizing the Middle East makes war more likely. A deal that provokes a nuclear arms race in the most volatile region on the globe makes war more likely. A deal that surrounds Israel not only with a nuclear Iran but also eventually with numerous other regimes with nuclear weapons capability and a genocidal attitude toward the Jewish State makes war more likely.
}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{JASA_paper/fig/TBIPhier_all/party_effects_interactions_k_15.pdf}
    \caption{Results of regression model with interactions built on ideological positions for topic~15.}
    \label{fig:TBIPhier_all_party_effects_interactions_k_15}
\end{figure}

\begin{comment}

\begin{enumerate}
    \item Additional covariates including interaction terms (gender, region, experience, generation).
    \item Table of estimated coefficients.
    \item Wordclouds and description of topics that are the most relevant wrt
    \begin{enumerate}
        \item gender - male vs female (beware of interaction with party)
        \item region - measure of discrepancy between 5 of those (e.g. stddev) 
        \item experience - newcomer vs more than 10 years of experience in Congress (skipping the middle group)
        \item generation - Silent vs Gen X (skipping the middle Boomers generation)
    \end{enumerate}
\end{enumerate}
\end{comment}



